Necessity Specifications for Robustness

Robust modules guarantee to do only what they are supposed to do - even in the presence of untrusted, malicious clients, and considering not just the direct behaviour of individual methods, but also the emergent behaviour from calls to more than one method. Necessity is a language for specifying robustness, based on novel necessity operators capturing temporal implication, and a proof logic that derives explicit robustness specifications from functional specifications. Soundness and an exemplar proof are mechanised in Coq.

==> adaptation.tex <==
\newsavebox\stateA
\newsavebox\stateB
\newsavebox\AadaptB

\newcommand{\extrasmall}[1]{{\fontsize{5pt}{6pt}#1}}

\begin{lrbox}{\stateA}
\begingroup
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{0.5} % Default value: 1
{\small$\sigma:$}
\begin{tabular}{l|l|l}
\textbf{\extrasmall{\prg{heap:}}}
&
\textbf{\extrasmall{\prg{local vars:}}}
&
\textbf{\extrasmall{\prg{contn:}}}\\
\begin{tabular}{l}
\extrasmall{\prg{a1}$\mapsto$\prg{o1}} \\
\extrasmall{\prg{a2}$\mapsto$\prg{o2}}
\end{tabular}
&
\begin{tabular}{l}
\extrasmall{\prg{this}$\mapsto$\prg{a1}} \\
\extrasmall{\prg{x}$\mapsto$\prg{a2}}\\
\extrasmall{\prg{y}$\mapsto$\prg{a2}}\\
\end{tabular}
&
\begin{tabular}{ll}
\extrasmall{\prg{1}} & \extrasmall{\prg{x:=5;}}\\
\extrasmall{\prg{2}} & \extrasmall{\prg{y.someMethod(x)}}\\
\extrasmall{\prg{3}} & \extrasmall{\prg{...}}
\end{tabular}
\end{tabular}
\endgroup
\end{lrbox}

\begin{lrbox}{\stateB}
\begingroup
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{0.5} % Default value: 1
{\small$\sigma':$}
\begin{tabular}{l|l|l}
\textbf{\extrasmall{\prg{heap:}}}
&
\textbf{\extrasmall{\prg{local vars:}}}
&
\textbf{\extrasmall{\prg{contn:}}}\\
\begin{tabular}{l}
\extrasmall{\prg{a1}$\mapsto$\prg{o1}} \\
\extrasmall{\prg{a2}$\mapsto$\prg{o2}}
\end{tabular}
&
\begin{tabular}{l}
\extrasmall{\prg{this}$\mapsto$\prg{a1}} \\
\extrasmall{\prg{x}$\mapsto$\prg{5}} \\
\extrasmall{\prg{y}$\mapsto$\prg{a2}}
\end{tabular}
&
\begin{tabular}{ll}
\extrasmall{\prg{1}} & \extrasmall{\prg{y.someMethod(x)}}\\
\extrasmall{\prg{2}} & \extrasmall{\prg{...}}
\end{tabular}
\end{tabular}
\endgroup
\end{lrbox}

\begin{lrbox}{\AadaptB}
\begingroup
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{0.5} % Default value: 1
{\small$\adapt{\sigma'}{\sigma}:$}
\begin{tabular}{l|l|l}
\textbf{\extrasmall{\prg{heap:}}}
&
\textbf{\extrasmall{\prg{local vars:}}}
&
\textbf{\extrasmall{\prg{contn:}}}\\
\begin{tabular}{l}
\extrasmall{\prg{a1}$\mapsto$\prg{o1}}\\
\extrasmall{\prg{a2}$\mapsto$\prg{o2}}
\end{tabular}
&
\begin{tabular}{l}
\extrasmall{\prg{this}$\mapsto$\prg{a1}} \\
\extrasmall{\prg{x}$\mapsto$\prg{a2}}\\
\extrasmall{\prg{y}$\mapsto$\prg{a2}}\\
\extrasmall{\prg{this'}$\mapsto$\prg{a1}} \\
\extrasmall{\prg{x'}$\mapsto$\prg{5}} \\
\extrasmall{\prg{y'}$\mapsto$\prg{a2}}
\end{tabular}
&
\begin{tabular}{ll}
\extrasmall{\prg{1}} & \extrasmall{\prg{y'.someMethod(x')}}\\
\extrasmall{\prg{2}} & \extrasmall{\prg{...}}
\end{tabular}
\end{tabular}
\endgroup
\end{lrbox}

\begin{tikzpicture}[->,>=to,shorten >=1pt,auto,node distance=7mm,
					decoration = snake]
\initialStateNode{\tiny{$\satisfies{\prg{MyMdl}, \sigma}{\access{\prg{this}}{\prg{x}}}$}}{A}{\usebox\stateA}; 
%\etcNode{blahA}{A};
\stateNode{\tiny{$\notsatisfies{\prg{MyMdl}, \sigma'}{\access{\prg{this}}{\prg{x}}}$}}{B}{right = of A}{\usebox\stateB};
\stateNode{\tiny{$\satisfies{\prg{MyMdl}, \adapt{\sigma'}{\sigma}}{\access{\prg{this}}{\prg{x}}}$}}{adapted}{below = of B}{\usebox\AadaptB};
	\draw [decorate, ->]
		(A) -- (B);
%	\draw [decorate, ->]
%		(blahA) -- (B);
\end{tikzpicture}


%\begin{minipage}{\textwidth}
%\begin{tabular}{cc}
%(A) &
%\begin{tikzpicture}[->,>=to,shorten >=1pt,auto,node distance=7mm,
%                    thick,
%                    external node/.style={circle,draw,minimum size=7mm,font=\sffamily\Large\bfseries, color=hotpink, fill = hotpink, text = black, fill opacity = 0.5},
%                    internal node/.style={circle,draw,minimum size=7mm,font=\sffamily\Large\bfseries, color=lightseagreen, fill = lightseagreen, text = black, fill opacity = 0.5},
%                    decoration = snake]
%    
%	\node[internal node] (a) {$\sigma_1$};
%	\node[external node] (b) [right = of a] {$\sigma_2$};
%	\node[internal node] (c) [right = of b] {$\sigma_3$};
%	\node[internal node] (d) [right = of c] {$\sigma_4$};
%	\node[external node] (e) [right = of d] {$\sigma_5$};
%	\node[external node] (f) [right = of e] {$\sigma_6$};
%	\node[internal node] (g) [right = of f] {$\sigma_7$};
%	\node[internal node] (h) [right = of g] {$\sigma_8$};
%	\node[external node] (i) [right = of h] {$\sigma_9$}; 
%
%%	\path[every node/.style={font=\sffamily\small}]
%%		(a) edge[left] node [above] {} (b)
%%		(b) edge[left] node [above] {} (c)
%%		(c) edge[left] node [above] {} (d)
%%		(d) edge[left] node [above] {} (e)
%%		(e) edge[left] node [above] {} (f)
%%		(f) edge[left] node [above] {} (g)
%%		(g) edge[left] node [above] {} (h)
%%		(h) edge[left] node [above] {} (i);
%
%	\draw [decorate, ->]
%	(a) -- (b);
%	\draw [decorate, ->]
%	(b) -- (c);
%	\draw [decorate, ->]
%	(c) -- (d);
%	\draw [decorate, ->]
%	(d) -- (e);
%	\draw [decorate, ->]
%	(e) -- (f);
%	\draw [decorate, ->]
%	(f) -- (g);
%	\draw [decorate, ->]
%	(g) -- (h);
%	\draw [decorate, ->]
%	(h) -- (i);
%\end{tikzpicture} \\
%%\end{tabular}
%%\end{minipage}
%%\begin{minipage}{\textwidth}
%%\begin{tabular}{cc}
%(B) &
%\begin{tikzpicture}[->,>=to,shorten >=1pt,auto,node distance=7mm,
%                    thick,
%                    external node/.style={circle,draw,minimum size=7mm,font=\sffamily\Large\bfseries, color=hotpink, fill = hotpink, text = black, fill opacity = 0.5},
%                    internal node/.style={circle,draw,minimum size=7mm,font=\sffamily\Large\bfseries, color=lightseagreen, fill = lightseagreen, text = black, fill opacity = 0.2, draw opacity = 0.5},
%                    decoration = snake,]
%    
%	\node[internal node] (a) {$\sigma_1$};
%	\node[external node] (b) [right = of a] {$\sigma_2$};
%	\node[internal node] (c) [right = of b] {$\sigma_3$};
%	\node[internal node] (d) [right = of c] {$\sigma_4$};
%	\node[external node] (e) [right = of d] {$\sigma_5$};
%	\node[external node] (f) [right = of e] {$\sigma_6$};
%	\node[internal node] (g) [right = of f] {$\sigma_7$};
%	\node[internal node] (h) [right = of g] {$\sigma_8$};
%	\node[external node] (i) [right = of h] {$\sigma_9$}; 
%
%%	\path[every node/.style={font=\sffamily\small}]
%%		(b) edge[left] node [above] {} (d)
%%		(d) edge[left] node [above] {} (e)
%%		(e) edge[left] node [above] {} (i);
%
%	\draw [decorate, ->]
%	(b) -- (e);
%	\draw [decorate, ->]
%	(e) -- (f);
%	\draw [decorate, ->]
%	(f) -- (i);
%\end{tikzpicture}
%\end{tabular}
%\end{minipage}

==> approach.lost.tex <==


\section{Outline of our approach}
\label{s:outline}
We now give an outline of our approach using a bank account example,   where funds may be transferred between accounts only if the account's password has been supplied.


 \subsection{Bank Account -- three modules}
\label{s:bank}
  
Module \prg{Mod1}   consists   of classes  \prg{Password} and  \prg{Account}
with a method called \prg{transfer}:
%
% (Note that we assume private fields are accessible ``class-wide''.)
%
% (methods may read and write fields of any instance of a class)
%
%and that passwords are unforgeable and not enumerable (again as
%in Java, albeit without reflection).
%
% 
\begin{lstlisting}[language=Chainmail, frame=lines]
module Mod1
  class Account
    field balance:int 
    field pwd: Password
    method transfer(dest:Account, pwd':Object) -> void
      if this.pwd==pwd'
        this.balance-=100
        dest.balance+=100
  class Password
\end{lstlisting}
%
\noindent 
We can capture the intended
semantics of % the \prg{transfer} method 
\prg{transfer} % by writing
through  a pre and postcondition 
JML-style\cite{Leavens-etal07}  ``classical''
specification, \sophiaPonder[]{-- all free variables are are universally quantified.}
\prg{Mod1}'s implementation of the \prg{transfer} method meets
this specification.



\begin{lstlisting}[mathescape=true, frame=lines, language=Chainmail]
ClassicBankSpec  $\triangleq$
   method transfer(dest:Account, pwd':Password) -> void {
       ( PRE:  this.balance=bal1 $\wedge$ this.pwd==pwd' $\wedge$ dest.balance=bal2 $\wedge$ dest=/=this 
         POST: this.balance == bal1-100 $\wedge$  dest.balance == bal2+100 )
       ( PRE: this.balance=bal1 $\wedge$ this.pwd=/=pwd' $\wedge$ dest.balance=bal2
         POST: this.balance == bal1 $\wedge$  dest.balance=bal2 )
       ( PRE: a : Account $\wedge$ a=/=this $\wedge$ a=/=dest  $\wedge$ a.balance=bal $\wedge$ a.pwd=pwd1
         POST:  a.balance=bal $\wedge$ a.pwd=pwd1)
       ( PRE: a : Account $\wedge$ a.pwd=pwd1  
         POST: a.pwd=pwd1)       
\end{lstlisting}
%\footnote{Perhaps omit some of the lines here, but we do need them all in the full discussion}
 
 

Now consider the following alternative implementations:
\prg{Mod2} allows any client to reset its password at any time, while
\prg{Mod3} first requires the existing password in order to change it.

%% The method \prg{transfer} in all three versions of the class \prg{Account} satisfies the (ClassicSpec), 
%% however, while executing the first and third version of \prg{Account} won't exhibit unwanted behaviour, the second version doesn't preclude it.
%Namely version II allows any client to change the password of the
%account, and then to repeatedly withdraw money from it.

  
% On the other hand, we expect our software -- even if complex -- to provide some simple, high level
%guarantees, e.g. email addressed to me personally will not be read by a third party unless I explicitly 
%forwarded it to them.
%We except  our software to  behave correctly, even when used by a careless or malicious third party. 
%Such use of a software often consist of a sequence of actions performed on the module. 
%
%Software components respond to single actions, 
%or to sequences of such single actions. 
%When thinking about a software component we want think about the behaviour of each 
%action in isolation, but also about the \emph{emergent behaviour}, ie all
% the possible effects of the combinations of these actions. 
  
  

\begin{tabular}{lll}
\begin{minipage}[b]{0.35\textwidth}
\begin{lstlisting}[language=chainmail, frame=lines]
module Mod2
  class Account
    field balance:int 
    field pwd: Password 
    method transfer(..) 
      ... as earlier ...
    method set(pwd': Object)
      this.pwd=pwd'
      
  class Password
\end{lstlisting}
\end{minipage}
&\ \ \  \ \   &%
\begin{minipage}[b]{0.50\textwidth}
\begin{lstlisting}[language=chainmail, frame=lines]
module Mod3
  class Account
    field balance:int 
    field pwd: Password 
    method transfer(..) 
      ... as earlier ...
    method set(pwd',pwd'': Object)
      if (this.pwd==pwd') 
        this.pwd=pwd''
  class Password
\end{lstlisting}
\end{minipage} 
\end{tabular}

Although the \prg{transfer} method is the same in
all three alternatives, and each one satisfies \prg{(ClassicBankSpec)},
code such as
%
\prg{account.set(42); account.transfer(yours, 42)}
%
are enough to drain the account in \prg{Mod2} without knowing the password.


 \subsection{Bank Account -- the right specification}
\label{s:bankSpecEx}

We need to rule out \prg{Mod2} while permitting \prg{Mod1} and
\prg{Mod3}. The catch is the vulnerability present in \prg{Mod2} is the result
of  \emph{emergent} behaviour from the interactions of the \prg{set}
and \prg{transfer} methods --- even though \prg{Mod3} also has a
\prg{set} method, it does not exhibit the unwanted interaction.
This is exactly where a necessary condition can help:
we want to avoid transferring money
(or more generally, reducing an account's balance)
\textit{without} the existing account password.  Phrasing the same condition
the other way around % gives us a positive statement that still
rules out the theft: that money \textit{can only} be
transferred when the account's password is known.
In \Nec  syntax:

%
%% The flaw in version {\sf{II}} arises from 
%% can be used to overwrite the
%% password, and then using the new password \prg{transfer}  can be called.
% If we want the \prg{Account} class to be robust, we must prohibit the password from being freely available.
%
%
%% In this paper, we show how \textit{necessity specifications} can solve
%% this progkem.  
%%  Therefore, we propose a %holistic 
%%  specification which says that
%%  the \prg{balance} of an \prg{Account} reduces only if an object which does not belong to the
%%  module has access to the password:
%
%
 %% Therefore, we propose a %holistic 
 %% specification which says that
 %% the \prg{balance} of an \prg{Account} reduces only if an object which does not belong to the
 %% module has access to the password:
%
\begin{lstlisting}[language = Chainmail, mathescape=true, frame=lines]
NecessityBankSpec  $\triangleq$   from a:Account $\wedge$ a.balance==bal
                        to a.balance < bal
                        onlyIf $\exists$ o.[$\external{\texttt{o}}$ $\wedge$ $\access{\texttt{o}}{\texttt{a.pwd}}$]
\end{lstlisting}
%
%
% 
%% In more detail, the specification from above says that if in the current
%% configuration \prg{a} is an \prg{Account},
%% and in some future configuration \prg{a} will have a balance less than the current one, then,in the \emph{current} configuration
%% there must exist some object \prg{o}, which is \emph{external} to our module (does not belong to module
 %% \prg{AccountMdl}), and which has access to \prg{a}'s password.
 %
%% T9hu having access to the password is a necessary condition for the balance to reduce.
The critical point of this \Nec specification is that it is
expressed in terms of observable effects and the shape of the heap --- the account's balance is reduced 
and there is external access to the password ($\external{\prg{o}}\ \wedge\ \access{\prg{o}}{\prg{a.pwd}}$)
--- and not in terms of individual methods --- such as
\prg{set} or \prg{transfer}.
This gives our specifications the
vital advantage that they constrain
\textit{implementation} of a bank account with a balance and a
password, irrespective of the API it
offers, the services it exports, or the dependencies on other parts of
the system.

%\sophiaPonder[skip that part?]
{This example also demonstrates that 
%the specification need  refer  to  individual methods in a module.
%Moreover, 
adherence to   \Nec specifications is not monotonic:
Adding a method to a module does not necessarily preserve adherence to a specification.
And while separate methods may adhere to a  specification, their combination does
not necessarily do so. Thus, \Nec specifications capture a module's \emph{emergent behaviour}. 
}

%\jm[TODO: in the proof later we need to mention that there is a difference between the overall proof (no mention of the methods), and the intermediate ones (that do mention the methods)]{}


%\subsection{Internal and External Modules, Objects, and Calls}

\subsection{Internal and External objects and calls}
\label{s:concepts}

Our work concentrates on guarantees made for the \emph{open} setting; that is, a given module
$M$ is programmed in such a robust manner
%\sophia[We had agreed no to say "robust", but I think it is OK here. Alternatively, say defensively robust?]{}
 that execution of $M$ together with \emph{any} \externalM 
module $M'$ will uphold these guarantees. In the tradition of
visible states semantics, we are  only interested in upholding the guarantees while 
$M'$, the  \externalM module,  is executing.   
 We therefore distinguish between \emph{\internalO} and
\emph{\externalO} objects: those that belong to classes defined in $M$, and the rest. Similarly, we 
distinguish between \emph{\internalC} calls, i.e. calls made % from \externalO objects
 to \internalO objects, and \emph{\externalC} calls, i.e. calls made % from \externalC objects
 to \externalC objects. % We are less
% interested in calls made from \internalO objects to \internalO objects, because we only need 
% establish the guarantees when the \externalM module is executing. And we 


Moreover, because we only require that the guarantees are upheld while 
  the  \externalM module  is executing, we develop an \emph{external states} semantics, where
 any internal calls are executed in one, large, step.
 Note that we do not -- yet -- support calls from
\internalO objects to \externalO objects.\sophia[we need to think where our system forbids that, ... ?]{} 
 With external steps semantics,  the executing object (the \prg{this}) is always   external. 
 


\subsection{Reasoning about Necessity}
\label{s:approach}
 
The proof that \prg{Mod3} adheres to \prg{NecessityBankSpec} consists,
broadly, of the following parts:


\begin{description}
\item[Part 1] We establish that  \textbf{(a)} the balance may only change through  
\prg{Mod3}-internal calls.
Also,  \textbf{(b)},   external accessibility to an account's password may 
only be obtained through  \prg{Mod3}-internal calls -- that is,  the property that
no external object has access to the password can only be invalidated through an internal call.
 
\item[Part 2] We establish  for each method of \prg{Mod3} (i.e. each method in \prg{Account} and \prg{Password}) that if the method is called, then 
 \textbf{(c)},  if it  causes the  balance to reduce, then the method called was
 \prg{transfer} and the correct password was provided, and 
  \textbf{(d)} it will not provide external accessibility to the password.

 \item[Part 3]  From \textbf{(a)}  and  \textbf{(c)} we obtain that \textbf{(e)}  if the balance were to 
reduce in \emph{any}  \emph{single} step -- whether an internal call, or any external step --
 the method called was
 \prg{transfer} and the correct password was provided. Similarly,   from
 \textbf{(b)}  and  \textbf{(d)} we obtain that \textbf{(f)}
 external accessibility to the password will not be provided by any single step.
    
 
\item[Part 4] From \textbf{(e)} we obtain that  \textbf{(g)}   if the balance reduces in any 
number of steps, then at some step  \prg{transfer} was called with   the correct password.
From  \textbf{(g)}  we obtain that \textbf{(h)} if the balance reduces in any 
number of steps, then at some intermediate step some external object had access to the password.
From \textbf{(f)} we obtain that  \textbf{(i)}  external accessibility to the password will not be provided by any sequence of steps.
Using  \textbf{(h)} and  \textbf{(i)}  we establish that
 \prg{Mod3} indeed adheres to \prg{NecessityBankSpec}.

\end{description} 
 
\noindent
We  now outline  the  formal concepts and ideas used in the four parts   from above:

\begin{description}
\item[Part 1] 
We  say assertion $A$  is
\emph{encapsulated} by  module $M$, if  $A$ can be invalidated only through
  $M$-\internalC calls. In short, an $M$-\internalC call is a \emph{necessary} condition for
invalidation of $A$.
% In \textbf{P1}, the assertion \prg{a:Account\! $\wedge$\! a.balance=bal} is encapsulated by \prg{Mod3}.

Determining encapsulation is a challenge, but not central to this work.
We therefore outline a rudimentary types-based algorithm, and relegate more
approaches to further work.
  
\item[Part 2]
 Here we infer a \emph{per-method-condition}, i.e., a 
 necessary condition given an effect and
a single, specified, method call. 
% 
%In \textbf{P2},   a necessary condition for the  reduction of \prg{a.balance}  after the call \prg{a.transfer(a',pwd)} is that the caller had access to \prg{a.password} before the call.

We address this  challenge % of the inference of necessary conditions 
 by leveraging the sufficient conditions from classical specifications:
If the negation of a method's
 classical postcondition implies  the effect we are interested in, then the negation of the 
 classical precondition  is the necessary precondition for the effect and the method call.
More in \S\ref{s:classical-proof}.  
 % Thus, 
 %  a method's sufficient conditions are used to infer a method's and effect's necessary conditions.



  
%\item[from effect and single step to necessary condition]
\item[Part 3]
Here we infer a \emph{per-step-condition}, i.e., a 
 necessary condition given an effect and
a single, unspecified step. This step could be an internal call, or any kind of external step.

%In \textbf{P3},   a necessary condition for the  reduction of \prg{a.balance}  after \emph{any}
%step, is that the caller  had access to \prg{a.password} before the call.
%And similarly in \textbf{P4},   a necessary condition for an external object's
%access to \prg{a.password}  after \emph{any}
%step, is that that object had access to \prg{a.password} before the call.

For effects encapsulated by $M$, we can infer such one-step
necessary conditions by combining the necessary conditions for that effect from 
all   methods in $M$. We also have  expected sub-structural rules, \emph{e.g.,} 
 like the rule of consequence.
More in \S\ref{s:module-proof}.



%\item[from effect to necessary conditions]
\item[Part 4]
  
We now infer the \emph{emergent} behaviour out of the many possible 
single steps.  This part is crucial;   remember that while \prg{Mod2} satisfies  
(***) for one single step, it does not satisfy it for any number of steps. More in \S\ref{s:emergent-proof}.
 
\end{description} 

\noindent
Note, that at no point do we inspect method bodies: we rely on type annotations
 to infer encapsulation, and on classical pre and post-conditions to infer per-method conditions.



==> approach_new.tex <==


\section{Outline of our approach}
\label{s:outline}

 \subsection{Bank Account -- three modules}
\label{s:bank}
  
Module \ModA consists of an empty 
\prg{Password} class where each instance models a unique password, and an  \prg{Account} class with a password, and a balance, an \prg{init} method to 
initialize the password, and 
a
\prg{transfer} method. 
%
% (Note that we assume private fields are accessible ``class-wide''.)
%
% (methods may read and write fields of any instance of a class)
%
%and that passwords are unforgeable and not enumerable (again as
%in Java, albeit without reflection).
%
% 
\begin{lstlisting}[mathescape=true, language=Chainmail, frame=lines]
module $\ModA$
  class Account
    field balance:int 
    field pwd: Password
    method transfer(dest:Account, pwd':Password) -> void
      if this.pwd==pwd'
        this.balance-=100
        dest.balance+=100
     method init(pwd':Password) -> void
      if this.pwd==null
        this.pwd=pwd'
  class Password
\end{lstlisting}
%
\noindent 
We can capture the intended
semantics of  
\prg{transfer}  
through  {a}  \funcSpec with pre- and postconditions as \emph{e.g.,} in \cite{Leavens-etal07,dafny13},
with ``explicit framing'' --   
 {rather than \prg{modifies}-clauses we give assertions   about preservation of values.}
 %\sophiaPonder[]{
%-- note that we always treat all free variables as universally quantified.
%}
\ModA's implementation of the \prg{transfer} method meets
this specification.



\begin{lstlisting}[mathescape=true, frame=lines, language=Chainmail]
$\Sclassic$  $\triangleq$
   method transfer(dest:Account, pwd':Password) -> void {
       ( PRE:  this.balance$=$bal1 $\wedge$ this.pwd$=$pwd' $\wedge$ dest.balance$=$bal2 $\wedge$ dest$\neq$this 
         POST: this.balance$=$bal1-100 $\wedge$  dest.balance$=$bal2+100 )
       ( PRE: this.balance$=$bal1 $\wedge$ this.pwd$\neq$pwd' $\wedge$ dest.balance=bal2
         POST: this.balance$=$bal1 $\wedge$  dest.balance$=$bal2 )
       ( PRE: a : Account $\wedge$ a$\neq$this $\wedge$ a$\neq$dest  $\wedge$ a.balance$=$bal
         POST:  a.balance$=$bal)
       ( PRE: a : Account $\wedge$ a.pwd$=$pwd1  
         POST: a.pwd$=$pwd1)       
\end{lstlisting}
%\footnote{Perhaps omit some of the lines here, but we do need them all in the full discussion}
 
 

Now consider the following alternative implementations:
\ModB allows any client to reset an account's password at any time;
\ModC requires the existing password in order to change it.
  
  

\begin{tabular}{lll}
\begin{minipage}[b]{0.42\textwidth}
\begin{lstlisting}[mathescape=true, language=chainmail, frame=lines]
module $\ModB$
  class Account
    field balance:int 
    field pwd: Password 
    method transfer(..) ...
      ... as earlier ...
    method init(...) ...
       ... as earlier ...
    method set(pwd': Password)
      this.pwd=pwd'
      
  class Password
\end{lstlisting}
\end{minipage}
&\ \ \  \ \   &%
\begin{minipage}[b]{0.45\textwidth}
\begin{lstlisting}[mathescape=true, language=chainmail, frame=lines]
module $\ModC$
  class Account
    field balance:int 
    field pwd: Password 
    method transfer(..) 
      ... as earlier ...
    
    
    method set(pwd',pwd'': Password)
      if (this.pwd==pwd') 
        this.pwd=pwd''
  class Password
\end{lstlisting}
\end{minipage} 
\end{tabular}

Although the \prg{transfer} method is the same in
all three alternatives, and each one satisfies \Sclassic,
code  {such as}
\\ 
$\ \strut \hspace{.2in} $ \prg{an\_account.set(42); an\_account.transfer(rogue\_account,42)}
\\ 
is enough to drain  \prg{an\_account} in \ModB without knowing the password.


 \subsection{Bank Account -- the right specification}
\label{s:bankSpecEx}

We \jm[]{need} a specification that rules out \ModB while permitting \ModA and
\ModC. The catch is that the vulnerability present in \ModB is the result
of  \emph{emergent} behaviour from the interactions of the \prg{set}
and \prg{transfer} methods --- even though \ModC also has a
\prg{set} method, it does not exhibit the unwanted interaction.
This is exactly where a necessary condition can help:
we want to avoid transferring money
(or more generally, reducing an account's balance)
\textit{without} the existing account password.  Phrasing the same condition
the other way around % gives us a positive statement that still
rules out the theft: that money \textit{can only} be
transferred when the account's password is known.


In \Nec  syntax, and {recalling section \ref{intro:this:work}, }
 

%
%% The flaw in version {\sf{II}} arises from 
%% can be used to overwrite the
%% password, and then using the new password \prg{transfer}  can be called.
% If we want the \prg{Account} class to be robust, we must prohibit the password from being freely available.
%
%
%% In this paper, we show how \textit{necessity specifications} can solve
%% this progkem.  
%%  Therefore, we propose a %holistic 
%%  specification which says that
%%  the \prg{balance} of an \prg{Account} reduces only if an object which does not belong to the
%%  module has access to the password:
%
%
 %% Therefore, we propose a %holistic 
 %% specification which says that
 %% the \prg{balance} of an \prg{Account} reduces only if an object which does not belong to the
 %% module has access to the password:
%
\begin{lstlisting}[language = Chainmail, mathescape=true, frame=lines]
   $\text{\SrobustA}$  $\triangleq$   from   a:Account $\wedge$ a.balance==bal    next    a.balance < bal
                onlyIf $\exists$ o,a'. [$\external{\prg{o}}$ $\wedge$ $\calls{\prg{o}}{\prg{a}}{\prg{transfer}}{\prg{a'},\prg{a.pwd}} $]    
                
   $\text{\SrobustB}$  $\triangleq$   from   a:Account $\wedge$ a.balance==bal    to    a.balance < bal
                onlyIf $\exists$ o.[$\external{\prg{o}}$ $\wedge$ $\access{\prg{o}}{\prg{a.pwd}}$]    
           
\end{lstlisting}
%
%
% 
%% In more detail, the specification from above says that if in the current
%% configuration \prg{a} is an \prg{Account},
%% and in some future configuration \prg{a} will have a balance less than the current one, then,in the \emph{current} configuration
%% there must exist some object \prg{o}, which is \emph{external} to our module (does not belong to module
 %% \prg{AccountMdl}), and which has access to \prg{a}'s password.
 %
%% T9hu having access to the password is a necessary condition for the balance to reduce.

 {Indeed, all three modules   satisfy  \SrobustA;  this demonstrates that \SrobustA is not
strong enough. On the other hand, \ModA and \ModC satisfy \SrobustB, while \ModB does not.  }

A critical point of \SrobustB % this \Nec specification 
is that it is
expressed in terms of observable effects (the account's balance is
reduced: \prg{a.balance < bal}) and the shape of the heap 
(external access to the password:
$\external{\prg{o}}\ \wedge\ \access{\prg{o}}{\prg{a.pwd}}$) 
rather than in terms of individual methods such as
\prg{set} and \prg{transfer}.
This gives our specifications the
vital advantage that they can be used to constrain
\jm[typo]{\textit{implementations}} of a bank account with a balance and a
password, irrespective of the API it
offers, the services it exports, or the dependencies on other parts of
the system.

 This example also demonstrates that 
adherence to   \Nec specifications is not monotonic:
adding a method to a module does not necessarily preserve adherence to
a specification, 
and while separate methods may adhere to a  specification, their combination does
not necessarily do so. 
{For example, \ModA satisfies \SrobustB, while \ModB does not.}
This is why we say that \Nec   specifications capture a module's \emph{emergent behaviour}. 
 

%\jm[TODO: in the proof later we need to mention that there is a difference between the overall proof (no mention of the methods), and the intermediate ones (that do mention the methods)]{}
\subsubsection{How applicable is  \SrobustB?}
\label{sec:how}
Finally,  {note that \SrobustB is applicable even though \emph{some} external objects may have access
to the account's password. 
Namely, if the account is passed to a scope which does not know the password, we 
know that its balance is guaranteed not to decrease. %, even though it may increase. 
}

 
We illustrate this through the following simplified code snippet.
 

\begin{lstlisting}[mathescape=true, language=chainmail, frame=lines]
module $\ModExt$
     ...
    method expecting_payment(untrusted:Object){ 
        a = new Account;
        p = new Password; 
        a.set(null,p);
        ...
        untrusted.make_payment(a);
        ...
    }
}
\end{lstlisting}
 

 The method \prg{expecting\_payment} has as  argument an external object \prg{untrusted}, of unknown provenance.
\sd{It} creates a new \prg{Account} and initializes its password. 

Assume that class \prg{Account} is from a module which satisfies \SrobustB. 
Then, 
in the scope of  method \prg{expecting\_payment} external objects have access to the password, 
and the balance may decrease  
during execution of  line 7, or   line \sd{9}. 
%\susan[Is this what you want to say? What if the code in line 8 does leak the password?
%\sd{I had errors in the lines. The code in line 8 cannot leak the password as it does not have it}]{}
However, if the code in line \sd{7} does not leak the password to \prg{untrusted}, then no external object
in  the scope of the call \prg{make\_payment} at line 8 has access to the password, and then,
even though we are calling   an untrusted object, \SrobustB guarantees that \prg{untrusted}
 will not be able to take any money out of  \prg{a}.
 
%\susan[I think this paragraph doesn't add, if anything it has a hostage to fortune. I would just remove it.
%\sd{agreed, and removed}]{}
% The purpose of the current paper is being able to express specifications like \SrobustB, and
%and being able to prove adherence. In further work we want to develop logics to leverage such specifications, putting
%informal arguments as the  one of this section onto formal foundations.
 

 
\subsection{Internal and External objects and calls}
\label{s:concepts}

Our work concentrates on guarantees made in an \emph{open} setting; that is, a given module
$M$ must be programmed so that %in such a robust manner
%\example[We had agreed no to say "robust", but I think it is OK here. Alternatively, say defensively robust?]{}
execution of $M$ together with \emph{any} \externalM 
module $M'$ will uphold these guarantees. In the tradition of
visible states semantics, we are  only interested in upholding the guarantees while 
$M'$, the  \emph{\externalM} module, is executing. A module can
temporarily break its own invariants,
%%just as a class or monitor can
%%break their invariants,
so long as the broken invariants are never visible externally.
   
We therefore distinguish between \emph{\internalO}
objects --- instances of classes defined in $M$ ---
and \emph{\externalO} objects defined in any other module, and
between \emph{\internalC} calls  (from either an internal or an external object)  made % from \externalO objects
 to \internalO objects and \emph{\externalC} calls made % from \externalC objects
 to \externalC objects. % We are less
% interested in calls made from \internalO objects to \internalO objects, because we only need 
% establish the guarantees when the \externalM module is executing. And we 
%
%
Because we only require guarantees while 
the  \externalM module  is executing,
we develop an \emph{external states} semantics, where
 any internal calls are executed in one, large, step.
With external steps semantics,  the executing object (\prg{this}) is always   external. 
Note that we do not support calls from
\internalO objects to \externalO objects.
 

\newcommand{\vertsp} {\vspace{.05in}} 
 
\subsection{Reasoning about Necessity}
\label{s:approach}
We now outline \sd{our  \Nec logic}.
We \sd{elaborate further} on the \jm[]{four} breakthroughs  \sd{described} \jm[]{in} %identified in 
\S\ref{intro:this:work}
along with two additions: (a) \funcSpecs, and (b) assertion encapsulation. 

 {Our logic  
 is based on the crucial insight that the specification $\onlyIf{A_1} {A_2} {A_3}$ is 
logically equivalent
% with 
{to}
 $\forall \prg{stmts}. \{ A_1 \wedge \neg A_3\} \prg{stmts} \{ \neg A_2 \}$ -- that is,
 with an infinite conjunction  of Hoare triples.}
 {This leaves the challenge that no Hoare logics support such infinite conjunctions.
 Three breakthroughs lead to our solution of that challenge:}
 \begin{description}
 \item
 [Per-method specs] 
  The Hoare triple 
$ \{ A_1 \wedge \neg A_3 \} \ \prg{x.m(ys)}\  \{ \neg A_2 \}$ is logically equivalent 
 {to} the specification
$ \onlyIfSingle {(A_1 \wedge  \calls{\_}{\prg{x}}{\prg{m}}{\prg{ys}} )} {A_2} {A_3}$.  
With this, we can leverage Hoare triples to reason about \sd{about any call  to one particular method }.  
 
 \item 
 [Per-step specs] % Second, 
 If an assertion $A_2$  is \emph{encapsulated} by a module (\ie the only way we can go from a 
 state that satisfies $A_2$ to a state that does not, is through a call to a method in that module), then
{the
\emph{finite conjunction}
of \sophiaPonder[moved negations]{$ \onlyIfSingle {(\, A_1 \wedge A_2 \wedge {\calls{\_}{\prg{x}}{\prg{m}}{\prg{ys}}}\, )} {\neg  A_2} {A_3}$}
 for all methods of that module is logically equivalent 
 {to}
 \sophiaPonder[moved negations]{$ \onlyIfSingle {A_1 \wedge A_2} {\neg A_2} {A_3}$. }}
  \item [Proof logic  for emergent behaviour] %an inference system 
  combines several specifications to reason about the
  emergent behaviour, \emph{e.g.,} 
   $ \onlyThrough  {A_1} {A_2} {A_3}$  and $ \onlyIf  {A_1} {A_3} {A_4}$ implies 
   $ \onlyIf  {A_1} {A_2} {A_4}$.
 \end{description}

%\jm[]{Julian Proposal >>>>>>>>>>>>>>>>>>>>>}


% and mentioned in \S \ref{intro:this:work} interact with each other.
%\jm[trimmed sentence]{} %to allow us to reason about 
%necessary conditions and emergent behaviour. 
%\Nec logic in this 
%paper is presented bottom up, starting with specifications of individual methods
%in isolation, building up to proofs of emergent behaviour.
%This section outlines the structure of 
%\Nec logic, and follows the 
\sophiaPonder[moved to earlier, so as to explain be more top-down]{
Our system} consists of four parts (five including \funcSpecs):
(\textbf{Part 1}) assertion encapsulation, (\textbf{Part 2}) \jm[]{per-method} specifications, 
(\textbf{Part 3}) per-step specifications, and (\textbf{Part 4}) specifications of emergent behaviour.
The structure of the system is given in Fig. \ref{fig:dependency}.
 \FuncSpecs are used to prove \jm[]{per-method} specifications, which coupled with 
assertion encapsulation is used to prove per-step specifications, which is used to 
prove specifications of emergent behaviour.
\begin{figure}[t]
\includegraphics[width=0.9\textwidth]{diagrams/dependency.png}
   \caption{
   Components of \Nec Logic \sd{and their Dependencies}. 
   Note that gray components with a dashed border indicate
   components that are not part of \Nec, and on which \Nec 
   is parametric.
    }
   \label{fig:dependency}
 \end{figure}

\jm[]{\Nec consists of specifications of necessary conditions and their proofs: parts 2, 3, and 4.
The remaining parts are assertion encapsulation (part 1) and \funcSpecs.}
An assertion $A$  is
\emph{encapsulated} by  module $M$, if  $A$ can be invalidated only through
calls to methods defined in $M$.
  In other words, a  call to  $M$  is a \emph{necessary} condition for
invalidation of $A$.
Our \Nec logic  is parametric with respect to the 
particular encapsulation
mechanism: examples in this paper rely on rudimentary annotations inspired by confinement types
\cite{confined}.
\jm[]{For the purposes of our examples,} \funcSpecs are assumed, and not 
included as part of the proof system, as they have been well covered in the literature.
{\jm[]{This is a key strength of our approach:
\Nec (parts 2, 3, and 4) and our results are } agnostic as to how \jm[]{both assertion encapsulation and} the pre- and post-conditions \jm[]{of the \funcSpecs} are proven.
As a result we can leverage the results of many different approaches.
Further, our proofs of \Nec do not inspect method
bodies: we rely on simple annotations to infer encapsulation, and
\sd{on} pre and post-conditions  to infer per-method conditions. }
 


 
%\jm[]{
%Note that our proofs of necessity do not inspect method
%bodies: we rely on simple annotations to infer encapsulation, and on
%classical pre and postconditions to infer per-method conditions. 
%{Our system is agnostic as to how the pre- and post-conditions are proven,
%and thus we can leverage the results of many different approaches.}
%}
%
%\jm[]{
%\begin{description}
%\item[Part 1: Assertion Encapsulation.] 
%An assertion $A$  is
%\emph{encapsulated} by  module $M$, if  $A$ can be invalidated only through
% % $M$-\internalC calls. 
%calls to methods defined in $M$.
%  In other words, a  call to  $M$  is a \emph{necessary} condition for
%invalidation of $A$.
%Our \Nec logic  is parametric with respect to the 
%particular encapsulation
%mechanism: here we rely on rudimentary annotations inspired by confinement types
%\cite{confined}. More in \S\ref{s:encaps-proof}.
%\item[Part 2: Per-method conditions]   % \emph{per-method-condition}, \ie., a 
%are derived using classical pre- and postconditions on methods.
%As we mention in \S \ref{intro:this:work}, the Hoare triple 
%$\{ A_1 \wedge \neg A_3 \} \ \prg{x.m(ys)}\  \{ \neg A_2 \}$
%is logically equivalent to stating that $A_3$ is a necessary precondition
%for the call \prg{x.m(ys)} with precondition $A_1$ to result in a postcondition $A_2$.
%More in \S\ref{s:classical-proof}.
%%are  necessary conditions for   given  effect and
%%  given single, specified, method call. 
%%To infer these, we  leverage   sufficient conditions 
%%from classical specifications: % Namely, if 
%%If the negation of a method's
%% classical postcondition implies  a given effect, %the effect we are interested in,
%%  then the negation of the 
%% classical precondition  is a necessary precondition for the effect and the method call. 
%%More in \S\ref{s:classical-proof}. 
% \item[Part 3: Single-step conditions] 
%If every method $m$ within a module $M$ has the same necessary condition, 
%$\onlyIfSingle{A \wedge \calls{\_}{x}{m}{ys}}{\neg A}{A_{necc}}$ (from Part 2), and 
%$A$ is encapsulated by $M$ (from Part 1), then it follows that $A_{necc}$ is a necessary precondition
%to invalidate $A$ for \emph{any} possible execution step.
%% are
%% necessary conditions for a given  effect and
%%a single, \emph{unspecified} step. This step could be an internal call, or any kind of external step.
%%    For effects encapsulated by $M$, we can infer such single-step
%% conditions by combining the per-method conditions for that effect from 
%%all   methods in $M$. 
%More in \S\ref{s:module-proof}.
%\item[Part 4: Emergent behaviour] \
%We infer the \emph{emergent} behaviour of a module out of the conditions of \sd{several}
%single steps (from Part 3) using a proof system defined in \S\ref{s:emergent-proof}.
%\end{description}
%}
%
%\jm[]{These parts are dependent on each other, along with an 
%assumed logic for proving classical pre- and postconditions.
%These dependencies are shown in Fig. \ref{fig:dependency}.}
 
For illustration, we  outline  a proof that  \ModC adheres to \SrobustB.
 
\begin{description}
\item[Part 1: Assertion Encapsulation.]  \
%
\vertsp\\
%
{\fbox{\parbox{\linewidth}{
We begin by proving that \ModC encapsulates: %3 properties:
\begin{description}
\item[(A)] The balance
\item[(B)] The password
\item[(C)] External accessibility to an account's password -- 
that is, the property that no external object has access to the password may only 
be invalidated by calls to \ModC.
\end{description}
}}}
% 
\vertsp
% 
\item[Part 2: Per-Method Specifications]   \
%
\vertsp\\
{\fbox{\parbox{\linewidth}{
\sd{We prove} that the call of any  method \sd{from} \ModC (\prg{set} and \prg{transfer}) 
satisfies: % is proven to have the following necessary conditions:
\begin{description}
\item[(D)] If the balance \sd{decreases}, then the method called was
 \prg{transfer} with the correct password
\item[(E)] If the password changes, then the method called was
 \prg{set} with the correct password
\item[(F)] It will not provide external accessibility to the password.
\end{description}
}}}
%
\vertsp
%
%
%
\item[Part 3: Per-step Specifications]  \
%
\vertsp \\ 
%
{\fbox{\parbox{\linewidth}{
We then raise our results of Parts 1 and 2 to reason about arbitrary \emph{single-step} executions:
\begin{description}
\item[(F)]
By \textbf{(A)} and \textbf{(D)} only \prg{transfer} and external knowledge of the password may decrease the balance.
\item[(G)]
By \textbf{(B)} and \textbf{(E)} only \prg{set} and external knowledge of the password may change the password.
\item[(H)]
By \textbf{(C)} and \textbf{(F)} no step may grant external accessibility to an account's password.
\end{description}
}}}
%
%\vertsp
%%
%{\fbox{\parbox{\linewidth}{
%Our proof that \textbf{(C2)} does not hold also considers single-step conditions, and takes the following form:
%\begin{description}
%\item[(G)]
%The internal-only access to an account's password is ``encapsulated'', and required internal computation to invalidate.
%\item[(H)]
%No internal method call can be used to coerce access to an account's password.
%\end{description}
%}}}
%  
\vertsp
%
\item[Part 4: Specifications of Emergent behaviour] \
%
\vertsp \\
%
{\fbox{\parbox{\linewidth}{
We then raise our necessary conditions of Part 3 to reason about \emph{arbitrary} executions:
\begin{description}
\item [(I)]
A decrease in balance over any number of steps implies that some single intermediate step 
reduced the account's balance.
\item [(J)] 
By \textbf{(F)} we know that step must be an external call to \prg{transfer} with the correct password.
\item [(K)]
When \prg{transfer} was called, either
\begin{description}
\item[(K1)]
The password used was the same as the current password, and thus by \textbf{(H)} we know that 
the current password must be externally known, satisfying \SrobustB, or
\item[(K2)] 
The password had been changed, and thus by \textbf{(G)} some intermediate step must have been
a call to \prg{set} with the current password. Thus, by \textbf{(H)} we know that
the current password must be externally known, satisfying \SrobustB.
\end{description}
\end{description}
}}}
%
\end{description}


%\noindent\jm[]{\noindent Original >>>>>>>>>>>>>>>>>>>>>}
%
%
%
%We now give a sketch of the novel concepts we developed in  \Nec logic.
%For illustration, we  outline  a proof that  \ModC adheres to \SrobustB.
%
%\begin{description}
%\item[Part 1: Emergent behaviour] \ {is behaviour that arises out 
%of any number of steps and interactions with a module interface.}
%We infer the \emph{emergent} behaviour out of the conditions of  \sd{several}
%single steps.
%This part is crucial;   \sd{for instance,} while \ModB satisfies  
%\SrobustB for one single step, it does not satisfy it for any number of steps. More in \S\ref{s:emergent-proof}.
%
%\vertsp
%%\jm{e.g. In the case of (S3) and \ModB, emergent behaviour refers to the interaction 
%%the \prg{set} method (for setting the password), the \prg{transfer} method, and the account's balance.}
%
%{\fbox{\parbox{\linewidth}{
%Our proof of \sd{\ModC's adherence to \SrobustB} follows the following steps:
%\begin{description}
%\item [(A)]
%A reduction in an account balance over any number of steps implies that some single intermediate step 
%reduced the account's balance.
%\item [(B)] 
%External knowledge of an account's password is a necessary prerequisite to any single step reducing the balance.
%\item [(C)]
%An account's password may only be externally known in the future if either
%\begin{description}
%\item[(C1)]
%the password is currently known externally  thus satisfying \SrobustB, or
%\item[(C2)] it is possible to coerce the internal module interface to expose the password
%\end{description}
%\end{description}
%The proof of (\textbf{B}) is constructed using \textbf{Part 2} and the proof that (\textbf{C2}) does not hold requires us to use the reasoning in \textbf{Part 2} and \textbf{Part 4}.
%}}}
%
%\vertsp 
%
% \item[Part 2: Single-step conditions] are
% necessary conditions for a given  effect and
%a single, \emph{unspecified} step. This step could be an internal call, or any kind of external step.
%  % 
%    For effects encapsulated by $M$, we can infer such single-step
% conditions by combining the per-method conditions for that effect from 
%all   methods in $M$. 
%% We also have  expected sub-structural rules,\eg  like the rule of consequence.
%% Drop above, as we dor 
%More in \S\ref{s:module-proof}.
%
%{\fbox{\parbox{\linewidth}{
%Our proof of \textbf{(B)} considers single-step conditions, and takes the following form:
%\begin{description}
%\item[(D)]
%An account's balance is an ``encapsulated'' property, that requires module internal computation to change.
%\item[(E)]
%The only module internal method call that reduces an account's balance is a call to \prg{transfer} with the account's 
%password.
%\item[(F)]
%An external call to \prg{transfer} with an account's password implies that the password is externally known
%\end{description}
%}}}
%
%\vertsp
%
%{\fbox{\parbox{\linewidth}{
%Our proof that \textbf{(C2)} does not hold also considers single-step conditions, and takes the following form:
%\begin{description}
%\item[(G)]
%The internal-only access to an account's password is ``encapsulated'', and required internal computation to invalidate.
%\item[(H)]
%No internal method call can be used to coerce access to an account's password.
%\end{description}
%}}}
% 
%\vertsp
% 
% 
%\item[Part 3: Per-method conditions]   % \emph{per-method-condition}, \ie., a 
%are  necessary conditions for   given  effect and
%  given single, specified, method call. 
%To infer these, we  leverage   sufficient conditions 
%from classical specifications: % Namely, if 
%If the negation of a method's
% classical postcondition implies  a given effect, %the effect we are interested in,
%  then the negation of the 
% classical precondition  is a necessary precondition for the effect and the method call. 
%More in \S\ref{s:classical-proof}. 
%
%\vertsp
%{\fbox{\parbox{\linewidth}{
%Our proofs of \textbf{(E)} and \textbf{(H)} take the following form:
%\begin{description}
%\item[(E)] Each method of \ModC (\ie each method in \prg{Account} and \prg{Password}),
%if it  causes the  balance to reduce, then the method called was
% \prg{transfer} and the correct password was provided
%\item[(H)] Each method of \ModC will not provide external accessibility to the password.
%\end{description}
%}}}
%
%  
%\vertsp
%
%
%\item[Part 4: Assertion Encapsulation.]  
%% \scd{We  introduce the concept} of  \emph{assertion  encapulation}: 
%% \scd{We define that an}
%An assertion $A$  is
%\emph{encapsulated} by  module $M$, if  $A$ can be invalidated only through
% % $M$-\internalC calls. 
%calls to methods defined in $M$.
%  In other words, a  call to  $M$  is a \emph{necessary} condition for
%invalidation of $A$.
%Our \Nec logic  is parametric with respect to the 
%particular encapsulation
%mechanism: here we rely on rudimentary annotations inspired by confinement types
%\cite{confined}.
%% In \textbf{P1}, the assertion \prg{a:Account\! $\wedge$\! a.balance=bal} is encapsulated by \ModC.
%%%%
%%%%Determining encapsulation is a challenge, but not central to this work.
%%%%We therefore outline a rudimentary types-based algorithm, and relegate more
%%%%approaches to further work.
%%%%
%
%\vertsp
%{\fbox{\parbox{\linewidth}{
%Our proofs of \textbf{(D)} and \textbf{(G)} take the following form:
%\begin{description}
%\item[(D)] The balance is encapsulated 
%by \ModC
%\item[(G)] External accessibility to an account's password may 
%only be obtained through calls to \ModC -- that is,  the property that
%no external object has access to the password is encapsulated by \ModC.
%\end{description}
%}}}
% 
%\end{description} 



%\scd{We now give a sketch of the   novel concepts we developed in  \Nec logic.
%For illustration, we  outline  a proof} that  \ModC adheres to \prg{NecessityBankSpec}.
%% we developoed in this work
%
%\begin{description}
%\item[Part 1: Assertion Encapsulation.]  
%% \scd{We  introduce the concept} of  \emph{assertion  encapulation}: 
%% \scd{We define that an}
%\scd{An} assertion $A$  is
%\emph{encapsulated} by  module $M$, if  $A$ can be invalidated only through
% % $M$-\internalC calls. 
% \scd{calls to methods defined in $M$}.
%  In other words, a  \sophiaPonder[said $M$-\internalC call]{call to  $M$}  is a \emph{necessary} condition for
%invalidation of $A$.
%\sophiaPonder[said: Our formalisation -- but I think what I say is stronger]{Our \Nec logic}  is parametric with respect to the 
%particular encapsulation
%mechanism: here we rely on rudimentary annotations inspired by confinement types
%\cite{confined}.
%% In \textbf{P1}, the assertion \prg{a:Account\! $\wedge$\! a.balance=bal} is encapsulated by \ModC.
%%%%
%%%%Determining encapsulation is a challenge, but not central to this work.
%%%%We therefore outline a rudimentary types-based algorithm, and relegate more
%%%%approaches to further work.
%%%%
%
%\vertsp
%
%For our proof, we establish that  \textbf{(a)} the balance is encapsulated 
%by \ModC, and  \textbf{(b)},   external accessibility to an account's password may 
%only be obtained through  \sophiaPonder[said: \ModC-internal] calls to \ModC -- that is,  the property that
%no external object has access to the password is encapsulated by \ModC.
%
%\vertsp
% 
% 
%\item[Part 2: Per-method conditions]   % \emph{per-method-condition}, \ie., a 
%are  necessary conditions for   given  effect and
%  given single, specified, method call. 
%To infer these, we  leverage   sufficient conditions 
%from classical specifications: % Namely, if 
%If the negation of a method's
% classical postcondition implies  \scd{a given effect}, %the effect we are interested in,
%  then the negation of the 
% classical precondition  is a necessary precondition for the effect and the method call. 
%More in \S\ref{s:classical-proof}. 
%
%\vertsp
%
%For our proof, we establish  for each method of \ModC (\ie each method in \prg{Account} and \prg{Password}) that if the method is called, then 
% \textbf{(c)},  if it  causes the  balance to reduce, then the method called was
% \prg{transfer} and the correct password was provided, and 
%  \textbf{(d)} it will not provide external accessibility to the password.
%  
%\vertsp
%
% 
%
% \item[Part 3: Single-step conditions] are
% necessary conditions for a given  effect and
%a single, \emph{unspecified} step. This step could be an internal call, or any kind of external step.
%  % 
%    For effects encapsulated by $M$, we can infer such single-step
% conditions by combining the per-method conditions for that effect from 
%all   methods in $M$. 
%% We also have  expected sub-structural rules,\eg  like the rule of consequence.
%% Drop above, as we dor 
%More in \S\ref{s:module-proof}.
% 
%\vertsp
%
%For our proof, from \textbf{(a)}  and  \textbf{(c)} we obtain that \textbf{(e)}  if the balance were to 
%reduce in \emph{any}  \emph{single} step -- whether an internal call, or any external step --
% the method called was
% \prg{transfer} and the correct password was provided. Similarly,   from
% \textbf{(b)}  and  \textbf{(d)} we obtain that \textbf{(f)}
% external accessibility to the password will not be provided by any single step.
% 
%\vertsp
%
% 
%\item[Part 4: Emergent behaviour] is the behaviour than can be observed by
%any number of steps. 
%We infer the \emph{emergent} behaviour out of the conditions of % many possible 
%single steps.  
%This part is crucial;   remember that while \ModB satisfies  
%(S3) for one single step, it does not satisfy it for any number of steps. More in \S\ref{s:emergent-proof}.
%
%\vertsp
%
%For our proof, from \textbf{(e)} we obtain that  \textbf{(g)}   if the balance reduces in any 
%number of steps, then at some step  \prg{transfer} was called with   the correct password.
%From  \textbf{(g)}  we obtain that \textbf{(h)} if the balance reduces in any 
%number of steps, then at some intermediate step some external object had access to the password.
%From \textbf{(f)} we obtain that  \textbf{(i)}  external accessibility to the password will not be provided by any sequence of steps.
%Using  \textbf{(h)} and  \textbf{(i)}  we establish that
% \ModC indeed adheres to \prg{NecessityBankSpec}.
% 
%\end{description} 
  
\noindent


  % Thus, 
 %  a method's sufficient conditions are used to infer a method's and effect's necessary conditions.

%\begin{description}
%\item[Part 1] We establish that  \textbf{(a)} the balance may only change through  
%\ModC-internal calls.
%Also,  \textbf{(b)},   external accessibility to an account's password may 
%only be obtained through  \ModC-internal calls -- that is,  the property that
%no external object has access to the password can only be invalidated through an internal call.
% 
%\item[Part 2] We establish  for each method of \ModC (\ie each method in \prg{Account} and \prg{Password}) that if the method is called, then 
% \textbf{(c)},  if it  causes the  balance to reduce, then the method called was
% \prg{transfer} and the correct password was provided, and 
%  \textbf{(d)} it will not provide external accessibility to the password.
%
% \item[Part 3]  From \textbf{(a)}  and  \textbf{(c)} we obtain that \textbf{(e)}  if the balance were to 
%reduce in \emph{any}  \emph{single} step -- whether an internal call, or any external step --
% the method called was
% \prg{transfer} and the correct password was provided. Similarly,   from
% \textbf{(b)}  and  \textbf{(d)} we obtain that \textbf{(f)}
% external accessibility to the password will not be provided by any single step.
%    
% 
%\item[Part 4] From \textbf{(e)} we obtain that  \textbf{(g)}   if the balance reduces in any 
%number of steps, then at some step  \prg{transfer} was called with   the correct password.
%From  \textbf{(g)}  we obtain that \textbf{(h)} if the balance reduces in any 
%number of steps, then at some intermediate step some external object had access to the password.
%From \textbf{(f)} we obtain that  \textbf{(i)}  external accessibility to the password will not be provided by any sequence of steps.
%Using  \textbf{(h)} and  \textbf{(i)}  we establish that
% \ModC indeed adheres to \prg{NecessityBankSpec}.
%
%\end{description} 
% 
%\noindent
%
%
%\begin{description}
%\item[Part 1] 
%We  say assertion $A$  is
%\emph{encapsulated} by  module $M$, if  $A$ can be invalidated only through
%  $M$-\internalC calls. In short, an $M$-\internalC call is a \emph{necessary} condition for
%invalidation of $A$.
%% In \textbf{P1}, the assertion \prg{a:Account\! $\wedge$\! a.balance=bal} is encapsulated by \ModC.
%%%%
%%%%Determining encapsulation is a challenge, but not central to this work.
%%%%We therefore outline a rudimentary types-based algorithm, and relegate more
%%%%approaches to further work.
%%%%
%Our formalisation is parametric with respect to the encapsulation
%mechanism: here we rely on rudimentary annotations inspired by confinement types
%\cite{confined}.
%  
%\item[Part 2]
% Here we infer a \emph{per-method-condition}, \ie., a 
% necessary condition given an effect and
%a single, specified, method call. 
%% 
%%In \textbf{P2},   a necessary condition for the  reduction of \prg{a.balance}  after the call \prg{a.transfer(a',pwd)} is that the caller had access to \prg{a.password} before the call.
%We address this  challenge % of the inference of necessary conditions 
% by leveraging the sufficient conditions from classical specifications:
%If the negation of a method's
% classical postcondition implies  the effect we are interested in, then the negation of the 
% classical precondition  is the necessary precondition for the effect and the method call.
%More in \S\ref{s:classical-proof}.  
% % Thus, 
% %  a method's sufficient conditions are used to infer a method's and effect's necessary conditions.



  
%\item[from effect and single step to necessary condition]

%In \textbf{P3},   a necessary condition for the  reduction of \prg{a.balance}  after \emph{any}
%step, is that the caller  had access to \prg{a.password} before the call.
%And similarly in \textbf{P4},   a necessary condition for an external object's
%access to \prg{a.password}  after \emph{any}
%step, is that that object had access to \prg{a.password} before the call.




%\item[from effect to necessary conditions]
 

%\noindent
%Note that our proofs of necessity do not inspect method
%bodies: we rely on simple annotations to infer encapsulation, and on
%classical pre and postconditions to infer per-method conditions. 
%{Our system is agnostic as to how the pre- and post-conditions are proven,
%and thus we can leverage the results of many different approaches.}


==> bankAccount.tex <==
\section{A Robust Bank Account}

\subsection{Traditional Bank Specification}

\subsection{Holistic Bank Specification}


==> coq.tex <==
\section{Coq Model}

\jm[]{As we have already mentioned in Section \ref{s:intro},
we include a Coq Model as suppelementary material to this paper.}


==> diagrams/necessity_operators_diagram.tex <==
\begin{figure}[htb]
\input{nec-diag}
   \caption{
   \Nec Operators
    }
   \label{fig:nec_operators}
 \end{figure}

==> introduction_old.tex <==
\section{Necessary Conditions and Robustness}
\label{s:intro}

%\subsection{Necessary conditions and Robustness}

%% Today's   software has been built 
%% over decades by combining modules and components of
%% different provenance and 
%% %different degrees of 
%% trustworthiness, and
%% is \emph{open}, interacting with other programs, devices, and people.

% according to IEEE standard,
% robust = The degree to which a system or component can function correctly in the presence 
% of invalid inputs or stressful environmental conditions.  

{Software needs} to be both {\emph{correct}} ({programs do what they
  are supposed to}) and {\emph{robust}} ({programs only do what
  they're supposed to}). Robustness means that
programs don't do what they aren't supposed to do, even in the
presence of untrusted or malicious {clients} \cite{ieeeStandard}.
% robust = The degree to which a system or component can function correctly in the presence 
% of invalid inputs or stressful environmental conditions.  
{Correctness is} classically specified
%formally 
through \citeasnoun{Hoare69} triples: a  precondition, a code snippet, and a
 postcondition. 
 For example,  {part of the classical specification
   of a \prg{transfer} method for a bank module is that the source account's balance decreases:}
 \begin{quote}
   \Scorrect\ \ $\triangleq$  
 % SD I could not make the below work ...
 % {\scriptsize \lstinline*{pwd=src.pwd  $\wedge$ \lstinline* src.bal=b} src.transfer(dst,pwd) {src.bal=b-100 * $\wedge$ \ldots } } }\\
 {\footnotesize{ $\{\,$\prg{pwd=src.pwd} $\,\wedge\,$ \prg{src.bal=b}$\,\}$ \prg{src.transfer(dst,pwd)} $\{$ \prg{src.bal=b-100}$\,\wedge\,\dots \}$ }} Calling \prg{transfer} on  {an account with the correct password} will transfer the money.
\end{quote}
Assuming termination, the precondition is a \emph{sufficient} condition for the {code snippet to behave correctly}: 
%assuming termination, 
the precondition (\eg providing the right 
password) guarantees that
the code (\eg call the \prg{transfer} function)
will always achieve the postcondition (the money is transferred).
 
    \vspace{.05in}
    % I think we need the vspace
 
%While 
\Scorrect  describes  {the \emph{correct use} of the module, but is \emph{not} concerned with its \emph{robustness}.}
{For example, can I pass an account to foreign untrusted code, in the expectation of receiving a payment,
but without fear that a malicious client might use the account to steal my money \cite{ELang}?}
 A first approach to specify robustness could be:
 

\begin{quote}
\SrobustA\ \ $\triangleq$ \ \ An account's balance does not decrease unless \prg{transfer} was called 
with the correct password.
\end{quote}

Specification \SrobustA % gives   the guarantee 
{guarantees} that it is not possible to  take money out of the account through some method other than \prg{transfer}
{or without providing the password}.
  Calling \prg{transfer}   with the  correct password is 
a \emph{necessary condition} for reducing the account's  balance.

\SrobustA is  crucial, but  not   enough:
it does not take  account of the module's \emph{emergent behaviour},
{that is, does not cater for the potential interplay of several methods offered by the module.}
 What if the module provided further methods which leaked the password,  
 {or allowed for it to be arbitrarily changed}?
{ While no single procedure call is capable of breaking the intent of \SrobustA, a sequence of calls might.}
{What} we really need is
 \begin{quote}
\SrobustB\ \ $\triangleq$ \ \ The balance of an account does not {\emph{ever}} decrease in the future unless some external 
object  {\emph{now}} has access to the account's current password.
\end{quote}
With \SrobustB, I can confidently pass my account to some untrusted client who
 does not have
 knowledge of the password; they may or may not make the payment I was expecting, but I
 know they will not  {be able to} steal my money \cite{ooToSecurity,miller-esop2013}.
 Note that \SrobustB  does not mention
 the names of any functions in the module, and 
 thus can be expressed without reference to any particular API ---
 indeed \SrobustB can constrain \emph{any} API with an account, an account
 balance, and a password.

\vspace{.04in}

 \subsection{{Earlier Work}} % SD I do not think this section is about robustness, since all the paper is about Robustness% Robustness is not a new idea, and anyway, this paper is also about robstness 
 

 %{\sd{Many} 
%kinds of} guarantees have been proposed\sophiaPonder[dropped: ``proposed for  robustness'']{}, differing in the level 
%of granularity,   target  language or calculi, and intended use.  
{Earlier work addressing robustness} includes object capabilities  \cite{MillerPhD, dd, threoremsFreeSep}, 
information control flow \cite{Zdancewic:Myers:01,noninteferenceOS}, 
 correspondence assertions \cite{Maffeis:aiamb:thesis00},
 sandboxing  \cite{robustSafetyPatrignani,sandbox},
robust linear temporal logic   \cite{RLTL2022} -- to name a few. %are some of the proposals to ensure some level of robust safety. 
{Most of these  %works 
propose \emph{generic} robustness guarantees (\emph{e.g.} no dependencies from high values to low values),
while we work with  \emph{problem-specific} guarantees  (\emph{e.g.} no decrease in balance without access to password).}
%
\Nec is the first approach that is able to  both express and prove
robustness specifications such as  \SrobustB.


{{\sc{VerX}} \cite{VerX} and  \emph{Chainmail} \cite{FASE} also work on problem-specific guarantees.}
Both these approaches can express necessary conditions
  like \SrobustA using
  temporal logic operators and implication. For example,  \SrobustA
 could be written as:
\\
 $\strut ~  ~ \hspace{.35in} \strut  \prg{a:Account} \ \wedge\ \prg{a.balance==bal}  \ \wedge\ 
\langle {\color{blue}\texttt{next}}\, \prg{a.balance<bal} \, \rangle $\\
 $\strut ~ \hspace{2.6in} \strut \strut \strut \longrightarrow\   \calls{\_}{\prg{a}}{\prg{transfer}}{\prg{\_,a.password}} $
 \\
\sophiaPonder[expalined and used similar syntax to below, and explained. But  now it get too too long :-(]{That is, if in the next state the balance of \prg{a} decreases, then the current state is 
a call to the method \prg{transfer} with the correct password passed. 
Note that  the underscore indicates
an existentially quantified variable used only once, for example,  $\calls{\_}{\prg{a}}{\prg{transfer}}{\prg{\_,a.password}}$
is short for $\exists \prg{o}.\exists \prg{a'}. \calls{\prg{o}}{\prg{a}}{\prg{transfer}}{\prg{a',a.password}}$. 
Here \prg{o} indicates the current receiver, i.e, the object whose method is currently being executed and making the call.
}

 {However, to express \SrobustB, one also needs what we call \emph{capability operators}, which talk about 
 provenance (``external object'') and
  permission (``\prg{x} has access to \prg{y}''). 
   {\sc{VerX}}  does not support capability operators, and thus cannot express   \SrobustB, 
   while  \emph{Chainmail} does support capability operators, and can express  \SrobustB. 
}  
 {\sc{VerX}} comes with a symbolic 
  execution system which can demonstrate adherence to its specifications, but doesn't have a proof logic, % to prove adherence,
   whereas, \emph{Chainmail}   {has neither a symbolic execution system, nor a proof logic.}
  % \susan[I have separated the tools rather than separating the features as I think it is clearer]{}
  
 {Temporal operators in {\sc{VerX}}   and  \emph{Chainmail}  are first class, \ie may appear in any assertions 
and form new assertions. This makes {\sc{VerX}}   and  \emph{Chainmail} very expressive,
and allows specifications which talk about any number of points in time.
However, this expressivity comes at the cost of making it very difficult to develop a logic to
prove adherence to such specifications.}
  
\vspace{.04in}

\subsection{\Nec}
\label{intro:this:work}
\Nec is a language for specifying a module's robustness guarantees 
and a logic 
to prove adherence to such specifications.

For the specification language we adopted  
\emph{Chainmail}'s    capability operators.
{For the 
  temporal operators, we observed that while their
   unrestricted combination with  other logical connectives allows us to talk about any
   number of points in time, the examples found in the literature talk about two or at most three such points. }

  
  {This led to the  crucial insight that we could merge  temporal operators and the implication 
 logical connective into our three}
   \emph{necessity} operators. 
 One such necessity operator is \\
$ 
\strut \hspace{1.7in} \onlyIf {A_{curr}} {A_{fut}} {A_{nec}}
$  
% \begin{lstlisting}[mathescape=true, language=chainmail, frame=lines]
%                                from ${A_{curr}}$ to ${A_{fut}}$ onlyIf ${A_{nec}}$ 
%\end{lstlisting}
%  %      $A$          from ${A_{curr}}$ to ${A_{fut}}$ onlyIf ${A_{nec}}$          from ${A_{curr}}$ to ${A_{fut}}$ onlyThrough ${A_{nec}}$
\\
This form says that  
a  {transition} from a current state satisfying assertion $A_{curr}$ to a future
state satisfying $A_{fut}$  is possible only if  the   necessary 
condition
$A_{nec}$ holds in the \emph{current} state.
Using this operator, we can formulate  \SrobustB  
as
\begin{lstlisting}[language = Chainmail, mathescape=true, frame=lines]
   $\text{\SrobustB}$  $\triangleq$   from   a:Account $\wedge$ a.balance==bal    to   a.balance < bal
               onlyIf  $\exists$ o.[$\external{\texttt{o}}$ $\wedge$ $\access{\texttt{o}}{\texttt{a.pwd}}$]
\end{lstlisting}
Namely, a transition from a  {current} state where an account's balance is \prg{bal}, to a  {future} state where 
it has decreased, may \emph{only} occur if  {in the current state} some unknown client object  
has access to that account's password. 
More discussion in \S\ref{s:bankSpecEx}. 


We also support two further \Nec operators:
\\
$ 
\strut \hspace{.4in} \onlyIfSingle {A_{curr}} {A_{fut}} {A_{nec}}. \strut \hspace{.4in} \onlyThrough {A_{curr}} {A_{fut}} {A_{intrm}}
$ 
\\
{The  first says    that 
a  \emph{one-step} {transition} from a current state satisfying assertion $A_{curr}$ to a future
state satisfying $A_{fut}$  
is possible only if % the   necessary condition
$A_{nec}$ holds in the \emph{current} state.   
The   second says that a change from %a current state satisfying 
 $A_{curr}$ to  $A_{fut}$  may happen only if % the necessary condition
 $A_{intrm}$ holds in some \emph{intermediate} state.}
 
  
  \vspace{.02in}
  
Unlike  \emph{Chainmail}'s temporal operators, 
 the necessity operators %  $\onlyIf {\_} {\_} {\_}$  and $\onlyThrough {\_} {\_} {\_}$
 are second class, and may not appear in the assertions  {(\eg  ${A_{curr}}$)}. 
 This simplification enabled us to develop our proof logic. 
 Thus, we {have reached} a  sweet spot between expressiveness and 
 provability.
 
We faced the challenge  how to develop a logic that would enable us to prove that code 
 adhered to  specifications {talking of system-wide properties.} 
 The Eureka moment was the realisation that all the information we required was hiding  { in the individual methods' classical specifications:}

 {Our logic  
 is based on the crucial insight that the specification $\onlyIf{A_1} {A_2} {A_3}$ is 
logically equivalent
% with 
{to}
 $\forall \prg{stmts}. \{ A_1 \wedge \neg A_3\} \prg{stmts} \{ \neg A_2 \}$ -- that is,
 with an infinite conjunction  of Hoare triples.}
 {This leaves the challenge that no Hoare logics support such infinite conjunctions.
 Three breakthroughs lead to our solution of that challenge:}
 \begin{description}
 \item
 [Per-method specs] 
  The Hoare triple 
$ \{ A_1 \wedge \neg A_3 \} \ \prg{x.m(ys)}\  \{ \neg A_2 \}$ is logically equivalent 
 {to} the specification
$ \onlyIfSingle {(A_1 \wedge  \calls{\_}{\prg{x}}{\prg{m}}{\prg{ys}} )} {A_2} {A_3}$.  
With this, we can leverage Hoare triples to reason about \sd{about any call  to one particular method }.  
 
 \item 
 [Per-step specs] % Second, 
 If an assertion $A_2$  is \emph{encapsulated} by a module (\ie the only way we can go from a 
 state that satisfies $A_2$ to a state that does not, is through a call to a method in that module), then
{the
\emph{finite conjunction}
of \sophiaPonder[moved negations]{$ \onlyIfSingle {(\, A_1 \wedge A_2 \wedge {\calls{\_}{\prg{x}}{\prg{m}}{\prg{ys}}}\, )} {\neg  A_2} {A_3}$}
 for all methods of that module is logically equivalent 
 {to}
 \sophiaPonder[moved negations]{$ \onlyIfSingle {A_1 \wedge A_2} {\neg A_2} {A_3}$. }}
  \item [Proof logic  for emergent behaviour] %an inference system 
  combines several specifications to reason about the
  emergent behaviour, \emph{e.g.,} 
   $ \onlyThrough  {A_1} {A_2} {A_3}$  and $ \onlyIf  {A_1} {A_3} {A_4}$ implies 
   $ \onlyIf  {A_1} {A_2} {A_4}$.
 \end{description}
  

\vspace{.02in}
\sophiaPonder[moved to earlier-I think fits better]{ }
Our work % formalization of \Nec  
{is 
parametric} with respect to assertion
satisfaction, encapsulation, and the type system.
We require  
classical specifications to have explicit framing.
{{Moreover, in line} with other work in the literature,} we forbid 
``callbacks'' out to  { \color{blue}\texttt{external}} objects (ie unknown objects
whose code has not been checked).   While our work is based on 
  a simple, imperative, typed, object oriented
language with unforgeable addresses and private fields, we believe
 that % our approach
 it is applicable to several programming paradigms, and 
 that   unforgeability and privacy
 can be replaced 
 by lower level mechanisms such as capability machines \cite{vanproving,davis2019cheriabi}.
 


\subsection{Paper Organization and Contributions}

%%In the next section, (\S\ref{s:outline}),  we outline our approach using a
%% bank account as  a motivating example.

%\jm[should this be ``a bank account''? This is the first time we mention it]{}
%
The contributions of this paper are:\begin{enumerate}
 \item
A language to
express \Nec specifications (\S\ref{s:semantics}).

 \item
A logic for proving a module's adherence to 
 \Nec specifications (\S\ref{s:inference}), and a proof of soundness of the logic, (\S\ref{s:soundness}),
both mechanized in Coq. 
 \item
A proof in our logic % the bank account 
  that our bank module obeys its \Nec specification (\S\ref{s:examples}),  also  mechanized in Coq.
\end{enumerate}


%\jm[]{
%Our formalization of \Nec does have two limitations. 
%Firstly, it is specifically a logic for 
%necessity and robustness properties. \Nec 
%is parametric with respect assertion satisfaction, correctness,
%encapsulation, and the type system. Much of these are
%well-trod ground in the literature, and where needed we
%do introduce simplistic language mechanisms to deal with them (e.g. a simple type system or notion of encapsulation).
%Secondly, we do not allow for ``callbacks'' 
%to external objects. This is a common restriction in the literature
%as many either prohibit callbacks, or require
%``effectively callback free contracts'' \cite{VerX},
%or place significant restrictions on callbacks \cite{}
%}


%We  discuss these  issues % limitations 
%further as 
\sophiaPonder[chopped "discuss issues"]{ } We place \Nec into the context of 
related work (\S\ref{s:related}) and consider our overall conclusions
(\S\ref{s:conclusion}). 
%
The Coq proofs of 
(2) and (3) above appear in the
supplementary material, along with \sd{a}ppendices containing expanded 
definitions and further examples.


==> toPutSomewhere.tex <==

% for the section on Spec^X

The first form says that $A$ always holds, \textit{i.e.} it is a invariant; 
it consists of assertions,  $A$, supporting the usual expressions about program state,
%%(e.g. \prg{x.f > 3}),
  logical connectives and quantifiers, 
%%(e.g. $\wedge$, $\forall$), 
 and additional predicates
 to capture \textit{provenance} and \textit{access}.
 %(whether an object $o$'s class comes 
%$\internal{\texttt{o}}$ or $\external{\texttt{o}}$) to the current
%module, and \textit{permission} \cite{miller-esop2013} (whether an
%object $o$ has direct access to another object $o'$:
%$\access{\texttt{o}}{\texttt{o'}}$).
The second form says that  a change from a current state satisfying $A_{curr}$ to a future
state satisfying $A_{fut}$ %(i.e.\ the transition  $A_{curr}$ to $A_{fut}$ being an effect) 
is possible only if the necessary condition
$A_{nec}$ holds in the current state.
%
%(i.e.\ $(A_1 \wedge \Diamond A_2) \longrightarrow A_3$).
The third form says that a change from a current state satisfying $A_{curr}$ to a future
state satisfying $A_{fut}$  is possible only if the necessary condition
$A_{nec}$ holds in some intermediate state.
 Note, that unlike \citeauthor{VerX} or \citeauthor{FASE}
 the necessity operators $\onlyIf {\_} {\_} {\_}$  and $\onlyThrough {\_} {\_} {\_}$
 are second class; they may nor appear in the assertions $A$.
 
 In section on proofs
  Thus, 
   a method's sufficient conditions are used to infer a method's and effect's necessary conditions.
 
 In section on compar with Verx
 \susan[logic sentence breaks flow and I would omit]{}$(A_1 \wedge \Diamond A_2) \longrightarrow A_3$ says that  $A_3$ is a necessary condition to
 transition from $A_1$ to $A_2$.
